ClusterFusion: Expanding Operator Fusion Scope for LLM Inference via Cluster-Level Collective Primitive

Large language model (LLM) decoding suffers from high latency due to fragmented execution across operators and heavy reliance on off-chip memory for data exchange and reduction. This execution model limits opportunities for fusion and incurs significant memory traffic and kernel launch overhead. While modern architectures such as NVIDIA Hopper provide distributed shared memory and low-latency intra-cluster interconnects, they expose only low-level data movement instructions, lacking structured abstractions for collective on-chip communication. To bridge this software-hardware gap, we introduce two cluster-level communication primitives, ClusterReduce and ClusterGather, which abstract common communication patterns and enable structured, high-speed data exchange and reduction between thread blocks within a cluster, allowing intermediate results to be on-chip without involving off-chip memory. Building on these abstractions, we design ClusterFusion, an execution framework that schedules communication and computation jointly to expand operator fusion scope by composing decoding stages such as QKV Projection, Attention, and Output Projection into a single fused kernels. Evaluations on H100 GPUs show that ClusterFusion outperforms state-of-the-art inference frameworks by 1.61x on average in end-to-end latency across different models and configurations. The source code is available at https://github.com/xinhao-luo/ClusterFusion.

==> sections/background.tex <==
\begin{figure}[htbp]
    \centering
    \begin{minipage}[t]{0.45\linewidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]{figs/llm.pdf}
        \caption{Typical Transformer Block as the fundamental component of the modern LLMs.}
        \label{fig:llm}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.54\linewidth}
        \centering
        \captionof{table}{Comparison of Prefill and Decode Latency at Different Sequence Lengths.}
        \label{tbl:pd}
        \resizebox{\linewidth}{!}{%
            \begin{tabular}{cccc}
                \toprule
                \textbf{Sequence Length} & \textbf{Prefill (s)} & \textbf{Decode 1 Token (s)} & \textbf{\% Time for Decoding 256 Tokens} \\
                \midrule
                1k   & 0.051  & 0.040 & 99.5\% \\
                4k   & 0.468  & 0.133 & 98.6\% \\
                16k  & 6.270  & 0.481 & 95.2\% \\
                \bottomrule
            \end{tabular}
        }
    \end{minipage}
\end{figure}

\section{Background}

% \subsection{LLM Inference Dataflow}
\subsection{\zhou{LLM Inference Workflow and Bottlenecks}}

% Mainstream LLMs are built upon the Transformer architecture. 
\zhou{Large language models (LLMs) are commonly built on transformer-based decoder-only architectures.}
As shown in \Fig{fig:llm}, each Transformer Block comprises Linear layers, Attention, and a Feed-Forward Network (FFN). For an input sequence \( X \), each attention head computes projections \( Q_i = XW_{Q_i}, \; K_i = XW_{K_i}, \; V_i = XW_{V_i} \), followed by scaled dot-product attention and output projection:

\begin{equation}
Z = \text{Concat}\left(\text{Softmax}\left(\frac{Q_1 K_1^\top}{\sqrt{d_k}}\right)V_1, \ldots, \text{Softmax}\left(\frac{Q_h K_h^\top}{\sqrt{d_k}}\right)V_h\right) W_O
\end{equation}

Here, \( d_k \) is the dimension of each head's Q and K. The FFN module applies three linear layers with a non-linear activation in between, formulated as:
\begin{equation}
\text{FFN}(Z) = W_3 \left( \sigma(W_1 Z) \odot W_2 Z \right)
\end{equation}
where \( \sigma \) is a non-linear activation (e.g., GELU), and \( \odot \) denotes element-wise multiplication. 

% In practice, most state-of-the-art LLMs adopt a decoder-only architecture, which generates output tokens sequentially using an auto-regressive pattern. The inference process is typically divided into two stages: prefill and decode.
\zhou{During inference, the model proceeds in two distinct stages: prefill and decode.}
During the prefill stage, the model processes the input prompt \zhou{in parallel to initialize} the key-value (KV) cache.
% , thereby initializing its internal memory. 
In the subsequent decode stage, \zhou{the model generates tokens one at a time in an auto-regressive manner, reusing the KV cache while appending new entries. This sequential decoding pattern inherently limits parallelism and dominates inference latency at longer context lengths.
As shown in \Tbl{tbl:pd}, decoding accounts for over 95\% of the total inference latency for 256-token sequences, as measured on SGLang~\cite{sglang}, a state-of-the-art LLM serving framework.
This makes decoding the dominant computational bottleneck during inference and a natural target for system-level performance optimization.
}
% the model generates one token at a time by consuming the most recent token along with the previously KV cache, and updates the cache with newly computed KV pairs. 
% This mechanism efficiently avoids redundant computations. 
% \Tbl{tbl:pd} presents a comparison of prefill and decode latencies at different sequence lengths, measured using state-of-the-art inference frameworks. The time required for decoding accounts for a substantial portion of the total inference time, especially as the sequence length grows. For example, at a sequence length of 16k tokens, the time required to decode a single token is much higher than at shorter sequence lengths, and the decoding process accounts for over 95\% of the total inference time for 256 tokens. 



\subsection{Existing Communication Patterns and Fusion Barriers}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/linattn.pdf}
    \caption{Existing Linear and Attention dataflow graph.}
    \label{fig:linattn}
\end{figure}

% In existing decoding dataflow designs, GPU thread blocks are typically used as the fundamental units of parallel execution. Each thread block operates independently, performing its assigned portion of the computation. 
\zhou{In existing GPU-based decoding dataflows, thread blocks serve as the fundamental unit of parallel execution and scheduling. This execution granularity governs how data is partitioned across blocks, how intermediate results are exchanged, and how operator fusion can be structured. Within each block, data dependencies are resolved using shared memory or registers, enabling local execution with efficient reuse of on-chip resources.}

% Typically, existing dataflow designs focus on using on-chip shared memory or registers to resolve intra-block data dependencies, enabling kernel fusion and reducing off-chip memory traffic. 

\zhou{\Fig{fig:linattn} illustrates an execution dataflow diagram extracted from XX’s decoding phase, where YY is invoked as the backend kernel. 
In this dataflow, the query vector $Q$ for a given token and attention head is broadcast to all thread blocks, while the key-value (KV) cache is partitioned across blocks along the sequence axis. Each block processes a disjoint segment of the KV cache and computes a partial attention result independently.
These partial results contribute to the same logical output and must be aggregated across thread blocks. This communication structure, in which multiple blocks produce partial results for a shared output, is commonly seen in attention~\cite{fa, flashinfer} and other reduction-style operations, such as the Split-K strategy in GEMM~\cite{cutlass?}. It creates inter-block data dependencies that must be coordinated during execution.
}
% As \Fig{fig:linattn} shows, a representative example is Flash-Decoding, where computation is parallelized along the KV cache token dimension due to the small Q token dimension during decoding. 
% In this dataflow, the same Q vector from a specific batch and attention head is replicated across multiple thread blocks, each responsible for processing a different slice of the corresponding KV cache. Each thread block computes partial results of the Attention. 



% A similar communication pattern appears in other dataflow, such as the Split-K dataflow in GEMM. In this approach, the reduction dimension (K) is partitioned into segments, each assigned to a different thread block, which computes a partial output by processing only its designated subset of the K dimension. These partial results correspond to the same output tile in the final matrix.

\zhou{
In current implementations, such dependencies are typically resolved through synchronization via global memory. Partial results are either accumulated using atomic operations, such as \textit{atomicAdd}, or written to memory and aggregated in a subsequent \textit{reduction} kernel. These synchronization mechanisms introduce off-chip memory traffic and fragment the decoding workflow across multiple kernel launches. As a result, operator fusion remains limited to intra-block execution, and all cross-block interactions require off-chip synchronization through global memory.
}
% In such designs, shared and register memory are used to stage intermediate results and resolve intra-block dependencies, such as $Q \times K^T$ and $Softmax$. However, inter-block data dependencies must rely on relatively slow global memory. Partial results are either written to global memory and aggregated by a subsequent reduction kernel, or directly accumulated into the same global memory address using operations such as $atomicAdd$. As with decoding and Split-K GEMM, these inter-block dependencies introduce global memory barrier for synchronization. This limits dataflow optimization to within individual kernels and results in redundant off-chip memory traffic, ultimately constraining the efficiency gains from fine-grained kernel fusion.

\subsection{Cluster-Level Opportunities and Challenges}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.33\linewidth]{figs/dsm_latency.pdf}
    \includegraphics[width=0.33\linewidth]{figs/dsm_throughput.pdf}
    \includegraphics[width=0.32\linewidth]{figs/dsm_sm.pdf}
    \caption{SM-to-SM access latency(left), throughput(middle) and the number of active SMs(right) for varying cluster size on NVIDIA Tesla H100 GPU.}
    \label{fig:dsm}
\end{figure}

\zhou{
1. intro cluster scope: opportunity
2. Hopper cluster/dsmem profiling: challenge
3. trend/other arch
}


\zhou{
As discussed in the previous section, existing GPU decoding workflows rely on global memory synchronization to resolve inter-block data dependencies. This limits the fusion scope to within individual thread blocks and restricts opportunities for structured execution across blocks. However, recent GPU architectures have introduced communication mechanisms that support fast data exchange within a thread block cluster, offering a new execution scope beyond the traditional block boundary.
}

As discussed in the previous section, existing GPU decoding workflows rely on global memory synchronization to resolve inter-block data dependencies. This limits the fusion scope to within individual thread blocks and restricts opportunities for structured execution across blocks. However, recent GPU architectures have introduced communication mechanisms that support fast data exchange within a thread block cluster, offering a new execution scope beyond the traditional block boundary. As a representative example, we briefly introduce the NVIDIA Hopper architecture, which incorporates such execution scope.

The NVIDIA Hopper architecture includes a direct, low-latency communication network between streaming multiprocessors (SMs) within a thread block cluster, which consists of 1 to 16 thread blocks. This design enables one thread block to access the shared memory of another block within the same cluster, a capability known as distributed shared memory (DSMEM). We profiled the DSMEM performance on the NVIDIA Tesla H100 GPU. As shown in \Fig{fig:dsm}, the SM-to-SM access latency reaches a minimum of 190 cycles at a cluster size of 2, while the corresponding throughput peaks at nearly 3.7 TB/s. For comparison, the access latency to global memory is approximately 450 cycles, L2 cache access latency is around 270 cycles, and transferring data between thread blocks through global memory incurs more than 900 cycles of latency. These results demonstrate that DSMEM offers significantly better performance, particularly in terms of latency. These results highlight the significant performance advantages of DSMEM, especially in terms of latency. While larger cluster sizes allow more thread blocks to leverage the shared memory, the throughput decreases, and the number of active SMs reduces as the cluster size increases, as depicted in \Fig{fig:dsm}. This reduction directly impacts parallelism and overall performance. Consequently, DSMEM performance exhibits a complex pattern, and finding the optimal configuration to balance it is essential.

Beyond Hopper, several other hardware architectures also support similar interconnect features. For example, the Cerebras Wafer-Scale Engine (WSE) is a wafer-level parallel compute accelerator containing a large number of processing elements interconnected through a two-dimensional mesh network. Similarly, AMD Radeon DNA (RDNA) architecture introduces a local data share mechanism, in which each workgroup processor is equipped with 128KB of memory, enabling low-latency communication between work-units within the same workgroup. However, research on leveraging the interconnect features to optimize modern LLM inference remains limited. Existing frameworks typically overlook the thread block cluster level and fail to incorporate performance optimizations that account for the complex characteristics of DSMEM.

==> sections/background_v2.tex <==
\begin{figure}[htbp]
    \centering
    \begin{minipage}[t]{0.45\linewidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]{figs/llm.pdf}
        \caption{Typical Transformer Block as the fundamental component of the modern LLMs.}
        \label{fig:llm}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.54\linewidth}
        \centering
        \captionof{table}{Comparison of Prefill and Decode Latency at Different Sequence Lengths.}
        \label{tbl:pd}
        \resizebox{\linewidth}{!}{%
            \begin{tabular}{cccc}
                \toprule
                \textbf{Sequence Length} & \textbf{Prefill (s)} & \textbf{Decode 1 Token (s)} & \textbf{\% Time for Decoding 256 Tokens} \\
                \midrule
                1k   & 0.051  & 0.040 & 99.5\% \\
                4k   & 0.468  & 0.133 & 98.6\% \\
                16k  & 6.270  & 0.481 & 95.2\% \\
                \bottomrule
            \end{tabular}
        }
    \end{minipage}
\end{figure}

\section{Background}

% \subsection{LLM Inference Dataflow}
\subsection{\zhou{LLM Inference Workflow and Bottlenecks}}

% Mainstream LLMs are built upon the Transformer architecture. 
\zhou{Large language models (LLMs) are commonly built on transformer-based decoder-only architectures.}
As shown in \Fig{fig:llm}, each Transformer Block comprises Linear layers, Attention, and a Feed-Forward Network (FFN). For an input sequence \( X \), each attention head computes projections \( Q_i = XW_{Q_i}, \; K_i = XW_{K_i}, \; V_i = XW_{V_i} \), followed by scaled dot-product attention and output projection:

\begin{equation}
Z = \text{Concat}\left(\text{Softmax}\left(\frac{Q_1 K_1^\top}{\sqrt{d_k}}\right)V_1, \ldots, \text{Softmax}\left(\frac{Q_h K_h^\top}{\sqrt{d_k}}\right)V_h\right) W_O
\end{equation}

Here, \( d_k \) is the dimension of each head's Q and K. The FFN module applies three linear layers with a non-linear activation in between, formulated as:
\begin{equation}
\text{FFN}(Z) = W_3 \left( \sigma(W_1 Z) \odot W_2 Z \right)
\end{equation}
where \( \sigma \) is a non-linear activation (e.g., GELU), and \( \odot \) denotes element-wise multiplication. 

% In practice, most state-of-the-art LLMs adopt a decoder-only architecture, which generates output tokens sequentially using an auto-regressive pattern. The inference process is typically divided into two stages: prefill and decode.
\zhou{During inference, the model proceeds in two distinct stages: prefill and decode.}
During the prefill stage, the model processes the input prompt \zhou{in parallel to initialize} the key-value (KV) cache.
% , thereby initializing its internal memory. 
In the subsequent decode stage, \zhou{the model generates tokens one at a time in an auto-regressive manner, reusing the KV cache while appending new entries. This sequential decoding pattern inherently limits parallelism and dominates inference latency at longer context lengths.
As shown in \Tbl{tbl:pd}, decoding accounts for over 95\% of the total inference latency for 256-tokens sequence, as measured using vLLM~\cite{sglang}, a state-of-the-art LLM serving framework.
This makes decoding the dominant computational bottleneck during inference and a natural target for system-level performance optimization.
}
% the model generates one token at a time by consuming the most recent token along with the previously KV cache, and updates the cache with newly computed KV pairs. 
% This mechanism efficiently avoids redundant computations. 
% \Tbl{tbl:pd} presents a comparison of prefill and decode latencies at different sequence lengths, measured using state-of-the-art inference frameworks. The time required for decoding accounts for a substantial portion of the total inference time, especially as the sequence length grows. For example, at a sequence length of 16k tokens, the time required to decode a single token is much higher than at shorter sequence lengths, and the decoding process accounts for over 95\% of the total inference time for 256 tokens. 



\subsection{Existing Communication Patterns and Fusion Barriers}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/linattn.pdf}
    \caption{Existing Linear and Attention dataflow graph.}
    \label{fig:linattn}
\end{figure}

% In existing decoding dataflow designs, GPU thread blocks are typically used as the fundamental units of parallel execution. Each thread block operates independently, performing its assigned portion of the computation. 
\zhou{In existing GPU-based decoding dataflows, thread blocks serve as the fundamental unit of parallel execution and scheduling. This execution granularity governs how data is partitioned across blocks, how intermediate results are exchanged, and how operator fusion can be structured. Within each block, data dependencies are resolved using shared memory or registers, enabling local execution with efficient reuse of on-chip resources.}

% Typically, existing dataflow designs focus on using on-chip shared memory or registers to resolve intra-block data dependencies, enabling kernel fusion and reducing off-chip memory traffic. 

\zhou{\Fig{fig:linattn} illustrates an execution dataflow diagram extracted from XX’s decoding phase, where YY is invoked as the backend kernel. 
In this dataflow, the query vector $Q$ for a given token and attention head is broadcast to all thread blocks, while the key-value (KV) cache is partitioned across blocks along the sequence axis. Each block processes a disjoint segment of the KV cache and computes a partial attention result independently.
These partial results contribute to the same logical output and must be aggregated across thread blocks. This communication structure, in which multiple blocks produce partial results for a shared output, is commonly seen in attention~\cite{fa, flashinfer} and other reduction-style operations, such as the Split-K strategy in GEMM~\cite{cutlass?}. It creates inter-block data dependencies that must be coordinated during execution.
}
% As \Fig{fig:linattn} shows, a representative example is Flash-Decoding, where computation is parallelized along the KV cache token dimension due to the small Q token dimension during decoding. 
% In this dataflow, the same Q vector from a specific batch and attention head is replicated across multiple thread blocks, each responsible for processing a different slice of the corresponding KV cache. Each thread block computes partial results of the Attention. 



% A similar communication pattern appears in other dataflow, such as the Split-K dataflow in GEMM. In this approach, the reduction dimension (K) is partitioned into segments, each assigned to a different thread block, which computes a partial output by processing only its designated subset of the K dimension. These partial results correspond to the same output tile in the final matrix.

\zhou{
In current implementations, such dependencies are typically resolved through synchronization via global memory. Partial results are either accumulated using atomic operations, such as \textit{atomicAdd}, or written to memory and aggregated in a subsequent \textit{reduction} kernel. These synchronization mechanisms introduce off-chip memory traffic and fragment the decoding workflow across multiple kernel launches. As a result, operator fusion remains limited to intra-block execution, and all cross-block interactions require off-chip synchronization through global memory.
}
% In such designs, shared and register memory are used to stage intermediate results and resolve intra-block dependencies, such as $Q \times K^T$ and $Softmax$. However, inter-block data dependencies must rely on relatively slow global memory. Partial results are either written to global memory and aggregated by a subsequent reduction kernel, or directly accumulated into the same global memory address using operations such as $atomicAdd$. As with decoding and Split-K GEMM, these inter-block dependencies introduce global memory barrier for synchronization. This limits dataflow optimization to within individual kernels and results in redundant off-chip memory traffic, ultimately constraining the efficiency gains from fine-grained kernel fusion.

\subsection{Cluster-Level Opportunities and Challenges}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.33\linewidth]{figs/dsm_latency.pdf}
    \includegraphics[width=0.33\linewidth]{figs/dsm_throughput.pdf}
    \includegraphics[width=0.32\linewidth]{figs/dsm_sm.pdf}
    \caption{SM-to-SM access latency(left), throughput(middle) and the number of active SMs(right) for varying cluster size on NVIDIA H100 GPU.}
    \label{fig:dsm}
\end{figure}

\zhou{
1. intro cluster scope: opportunity
2. Hopper cluster/dsmem profiling: challenge
3. trend/other arch/fraework， hopper-soution is lacking
}

\zhou{
As discussed in the previous section, existing GPU decoding workflows rely on global memory synchronization to resolve inter-block data dependencies. 
Recent architectures, such as NVIDIA Hopper, introduce hardware support for intra-cluster coordination through the thread block cluster abstraction. Within a cluster, multiple thread blocks can exchange data using distributed shared memory (DSMEM), enabling cross-block interaction without global memory.
}

% As discussed in the previous section, existing GPU decoding workflows rely on global memory synchronization to resolve inter-block data dependencies. This limits the fusion scope to within individual thread blocks and restricts opportunities for structured execution across blocks. However, recent GPU architectures have introduced communication mechanisms that support fast data exchange within a thread block cluster, offering a new execution scope beyond the traditional block boundary. As a representative example, we briefly introduce the NVIDIA Hopper architecture, which incorporates such execution scope.

% The NVIDIA Hopper architecture includes a direct, low-latency communication network between streaming multiprocessors (SMs) within a thread block cluster, which consists of 1 to 16 thread blocks. This design enables one thread block to access the shared memory of another block within the same cluster, a capability known as distributed shared memory (DSMEM). 


\zhou{To understand the opportunities and challenges of this mechanism, we profile DSMEM on an NVIDIA H100 GPU by varying the cluster size from 1 to 16, which is the maximum supported by Hopper hardware.
As shown in \Fig{fig:dsm}, SM-to-SM access latency improves significantly with small cluster sizes. When the cluster size is 2, the average latency reaches 190 cycles, which is substantially lower than global memory latency (exceeding 900 cycles). This demonstrates the potential of DSMEM for low-latency on-chip communication.

However, this benefit comes with notable trade-offs. As the cluster size increases, the available communication bandwidth decreases, and the number of active SMs is reduced due to hardware constraints. These effects limit the scalability of cluster-based execution and necessitate careful configuration to balance communication efficiency and overall parallelism.

Beyond hardware-level trade-offs, there are software-level challenges as well. 
NVIDIA currently exposes DSMEM and thread block cluster functionality only through low-level PTX instructions, which only support basic peer-to-peer data movement but lack higher-level communication primitives. This creates a high programming barrier and provides no standardized way to orchestrate collective execution across thread blocks.
% Fully exploiting the cluster execution scope requires software abstractions that enable collective coordination across thread blocks while respecting the underlying hardware constraints. 

Similar interconnect capabilities have been adopted in other hardware platforms, including AMD RDNA and Cerebras WSE, reflecting a broader trend toward enabling on-chip coordination across compute units.
T10...
WaferLLM...
However, system-level solutions that effectively utilize the DSMEM communication model on Hopper GPUs remain absent. 
Hopper Feature...
}
% Similar interconnect mechanisms have also been adopted in other architectures, including AMD RDNA~\cite{}, Cerebras WSE~\cite{}, and XXX~\cite{}, which support low-latency on-chip inter-core coordination. This trend underscores the broader relevance of structured cluster-level execution beyond a single platform. 

% We profiled the DSMEM performance on the NVIDIA Tesla H100 GPU. 
% As shown in \Fig{fig:dsm}, the SM-to-SM access latency reaches a minimum of 190 cycles at a cluster size of 2, while the corresponding throughput peaks at nearly 3.7 TB/s. For comparison, the access latency to global memory is approximately 450 cycles, L2 cache access latency is around 270 cycles, and transferring data between thread blocks through global memory incurs more than 900 cycles of latency. These results demonstrate that DSMEM offers significantly better performance, particularly in terms of latency. These results highlight the significant performance advantages of DSMEM, especially in terms of latency. However, NVIDIA expose only low-level data movement instructions, lacking structured abstractions for using in real workload. This results in a steep programming barrier and leaves developers without clear guidance on how to effectively apply these capabilities. Furthermore, our profiling reveals that DSMEM performance is highly sensitive to cluster configuration and access patterns, making it difficult to optimize communication using only raw instructions.

% Beyond Hopper, several other hardware architectures also support similar interconnect features. For example, the Cerebras Wafer-Scale Engine is a wafer-level parallel compute accelerator containing a large number of processing elements interconnected through a two-dimensional mesh network. Similarly, AMD Radeon DNA 3 architecture introduces a local data share mechanism, in which each workgroup processor is equipped with 128KB of memory, enabling low-latency communication between work-units within the same workgroup. However, research on leveraging the interconnect features to optimize modern LLM inference remains limited. Existing frameworks typically overlook the thread block cluster level and fail to incorporate performance optimizations that account for the complex characteristics of DSMEM.

==> sections/design.tex <==
\section{ClusterFusion: Cluster-Aware Decoding Fusion}

In this section, we introduce ClusterFusion, a cluster-aware decoding fusion dataflow. We begin by outlining its execution model and core design principles. Next, we demonstrate how low-latency DSMEM can be leveraged to implement efficient cluster-scoped communication primitives. Finally, we present the unified cluster-aware decoding dataflow with these primitives.

\begin{figure}[htbp]
    \centering
    \subcaptionbox{ClusterReduce\label{fig:api_reduce}}{\includegraphics[width=0.49\linewidth]{figs/all-reduce.pdf}}
    \subcaptionbox{ClusterGather\label{fig:api_gather}}{\includegraphics[width=0.49\linewidth]{figs/all-gather.pdf}}
    \caption{Cluster-Level Collective Communication Primitives: ClusterReduce and ClusterGather}
    \label{fig:api}
\end{figure}

\subsection{Execution Model and Design Principles}

\subsection{Cluster-Level Collective Communication Primitives}
\label{sec:api}

\begin{algorithm}[]
    \caption{ClusterReduce over DSMEM - Thread Block view}
    \label{alg:cluster_reduce}
    \begin{algorithmic}[1]
    \Require
    A cluster of $N = 2^k$ thread blocks ($k \leq 4$), each with rank $b \in [0, N-1]$ and a shared memory buffer $\mathbf{D}_b$ containing local data that needs to be reduced together with data from other thread blocks in the same cluster.
      % DSMEM enables inter-block communication within the cluster
    % \Ensure
      % Each $\mathbf{D}_b$ contains $\sum_{j=0}^{N-1} \mathbf{D}_j$
    \State Initialize shared memory buffer $\mathbf{B}_b$ with the same size of $\mathbf{D}_b$ \Comment{Used as a temporary buffer}.
    \State $\texttt{stride} \gets 1$.
    \While{$\texttt{stride} < N$}
        \State block rank $\texttt{send\_to} \gets (b + \texttt{stride}) \bmod N$.
        \State block rank $\texttt{recv\_from} \gets (b - \texttt{stride} + N) \bmod N$.
        \State Send $\mathbf{D}_b$ to $\mathbf{B}_{\texttt{send\_to}}$ of block $\texttt{send\_to}$ via DSMEM.
        \State Receive $\mathbf{D}_{\texttt{recv\_from}}$ from block $\texttt{recv\_from}$ into $\mathbf{B}_b$ via DSMEM.
        \State Wait for the arrival of $\mathbf{D}_{\texttt{recv\_from}}$.
        \State $\mathbf{D}_b \gets \mathbf{D}_b \oplus \mathbf{B}_{b}$ \Comment{Aggregate partial result using a reduction operator $\oplus$ (e.g., sum or max)}
        \State $\texttt{stride} \gets \texttt{stride} \times 2$ \Comment{Exponential stride progression}
    \EndWhile
    \State Return $\mathbf{D}_b$. 
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[]
    \caption{ClusterGather over DSMEM - Thread Block view}
    \label{alg:cluster_gather}
    \begin{algorithmic}[1]
    \Require
    A cluster of $N = 2^k$ thread blocks ($k \leq 4$), each with rank $b \in [0, N-1]$ and a shared memory buffer $\mathbf{D}_b$ of size $N \times \texttt{size}$. The first segment $\mathbf{D}_b[0:\texttt{size}]$ contains the local data that needs to be gathered together with data from other thread blocks in the same cluster.
      % DSMEM enables inter-block communication within the cluster
    % \Ensure
      % Each $\mathbf{D}_b$ contains $\sum_{j=0}^{N-1} \mathbf{D}_j$
    \State $\texttt{stride} \gets 1$.
    \While{$\texttt{stride} < N$}
        \State block rank $\texttt{send\_to} \gets (b + \texttt{stride}) \bmod N$.
        \State block rank $\texttt{recv\_from} \gets (b - \texttt{stride} + N) \bmod N$.
        \State Send $\mathbf{D}_b[0:\texttt{size} \times \texttt{stride}]$ to $\mathbf{D}_{\texttt{send\_to}}[\texttt{stride} \times \texttt{size} : 2 \times \texttt{stride} \times \texttt{size}]$ of block $\texttt{send\_to}$ via DSMEM.
        \State Receive $\mathbf{D}_{\texttt{recv\_from}}[0:\texttt{size} \times \texttt{stride}]$ from block $\texttt{recv\_from}$ into $\mathbf{D}_b[\texttt{stride} \times \texttt{size} : 2 \times \texttt{stride} \times \texttt{size}]$ via DSMEM.
        \State Wait for the arrival of $\mathbf{D}_{\texttt{recv\_from}}[0:\texttt{size} \times \texttt{stride}]$.
        \State $\texttt{stride} \gets \texttt{stride} \times 2$ \Comment{Exponential stride progression}
    \EndWhile
    \State Return $\mathbf{D}_b$. 
    \end{algorithmic}
\end{algorithm}

\zhou{
1. intro NV existing DSMEM/Cluster API/capabilities
2. clear state existing API cannot address challenge
3. present overall goals of primitive
}

As clusters enable inter-thread block communication to resolve data dependencies across blocks, they open up new optimization opportunities. However, our profiling reveals that DSMEM performance varies significantly with different cluster configurations and requires careful tuning. Moreover, the current use of DSMEM lacks standardized approaches. To address this, we propose a set of general communication primitives that leverage DSMEM to resolve on-chip block-level data dependencies. These primitives are designed to be compatible with various cluster configurations and can be directly tuned for performance.

On the NVIDIA Hopper architecture, we abstract the thread block cluster as a low-latency, fully connected network, with each thread block treated as an individual node. Leveraging this abstraction, we design customized cluster-level collective communication primitives: ClusterReduce and ClusterGather. As illustrated in \Fig{fig:api}, ClusterReduce aggregates partial data from all nodes by summing them and then redistributes the result back to each node. In contrast, ClusterGather transmits the local data of each node to all others, so that every node holds a complete replica of the combined data after the operation completes.

As described in \Alg{algo:api}, the on-chip ClusterReduce and ClusterGather collective communication primitives share a structurally similar communication pattern based on a binary tree topology. Both algorithms operate over $\log_2 N$ rounds, where each block communicates with a partner determined by an exponentially growing stride - first with adjacent blocks (stride 1), then every second block (stride 2), followed by every fourth block (stride 4), and so forth. ClusterReduce maintains strict data size throughout all communication rounds, using element-wise operations such as summation or maximization to merge received data with local values. In contrast, ClusterGather adopts an opposing approach where each round doubles the exchanged data volume through simple buffer concatenation.

\begin{algorithm}[]
    \caption{Decoding Fusion Dataflow for LLaMA MHA Architecture - Thread Block View}
    \label{alg:llama_fusion}
    \begin{algorithmic}[1]
    \Require
    Input hidden states $\mathbf{H}_b \in \mathbb{R}^{B \times d}$, linear-QKV weight $\mathbf{W}^{QKV}_b \in \mathbb{R}^{d \times 3h}$, output projection weight $\mathbf{W}^O_b \in \mathbb{R}^{h \times d}$, and KV cache $\mathbf{K}^{\text{cache}}_b, \mathbf{V}^{\text{cache}}_b \in \mathbb{R}^{s \times h}$ in global memory.

    \State Allocate shared memory buffers: $\mathbf{Q}_b, \mathbf{K}_b, \mathbf{V}_b \in \mathbb{R}^{B \times h}$, and $\mathit{Softmax}_{\text{sum}}, \mathit{Softmax}_{\text{max}}$.

    \State Compute partial results of fused linear projection: 
    \[
        \mathbf{Q}_b, \mathbf{K}_b, \mathbf{V}_b \gets \mathbf{H}_b \times \mathbf{W}^{QKV}_b
    \]

    \State Apply \texttt{ClusterReduce} primitives to obtain the complete $\mathbf{Q}_b, \mathbf{K}_b, \mathbf{V}_b$:
    \[
        (\mathbf{Q}_b, \mathbf{K}_b, \mathbf{V}_b) \gets \texttt{ClusterReduce}(\mathbf{Q}_b, \mathbf{K}_b, \mathbf{V}_b)
    \]

    \State Compute partial result of attention with FlashDecoding dataflow:
    \[
        \mathbf{A}_b \gets \texttt{FlashDecoding}(\mathbf{Q}_b, \mathbf{K}_b, \mathbf{V}_b, \mathbf{K}^{\text{cache}}_b, \mathbf{V}^{\text{cache}}_b)
    \]
    and obtain local statistics $\mathit{Softmax}_{\text{sum}}, \mathit{Softmax}_{\text{max}}$. \Comment{$\mathbf{A}_b$ can reuse the shared memory of $\mathbf{Q}_b$}

    \State Store $\mathit{Softmax}_{\text{max}}$ in register: $\mathit{Reg}_{\text{max}} \gets \mathit{Softmax}_{\text{max}}$.

    \State Apply \texttt{ClusterReduce} primitives to obtain the complete $\mathit{Softmax}_{\text{sum}}$ and $\mathit{Softmax}_{\text{max}}$:
    \[
        \mathit{Softmax}_{\text{sum}} \gets \texttt{ClusterReduce}(\mathit{Softmax}_{\text{sum}}), 
    \]
    \[
        \mathit{Softmax}_{\text{max}} \gets \texttt{ClusterReduce}(\mathit{Softmax}_{\text{max}})
    \]

    \State Rescale attention output according to online softmax:
    \[
        \mathbf{A}_b \gets \frac{\mathbf{A}_b \cdot \exp(\mathit{Reg}_{\text{max}} - \mathit{Softmax}_{\text{max}})}{\mathit{Softmax}_{\text{sum}}}
    \] \Comment{This is analogous to performing a local softmax in each block and rescaling to obtain the final result.}

    \State Apply \texttt{ClusterReduce} primitives to obtain the complete $\mathbf{A}_b$:
    \[
        \mathbf{A}_b \gets \texttt{ClusterReduce}(\mathbf{A}_b)
    \]

    \State Compute the result of the output projection and write it to global memory using \texttt{atomicAdd}: 
    \[
        \mathbf{O}_b \gets \mathbf{A}_b \times \mathbf{W}^O_b
    \]

    \State \Return $\mathbf{O}_b$.
    \end{algorithmic}
\end{algorithm}

\subsection{Unified Dataflow with Cluster-Level Primitives}
% \subsection{Cluster-Centric Pipeline Programming with Primitives}

The computation dataflow in the decoding stage is parallelized across different dimensions for the linear and attention layers. Specifically, the linear layer is parallel along the hidden and output dimensions, while the attention layer is parallel across the number of attention heads and the KV cache sequence length. Among these dimensions, thread blocks that compute different partitions of the output dimension and the KV sequence length have data dependencies, as each block generates a partial result that must be reduced to produce the final output. These dependent thread blocks can be organized into a cluster. Under this design, the intermediate results produced by the linear stage naturally reside on chip and directly satisfy the data dependency requirements of the attention stage. This enables the two stages to be seamlessly fused via shared memory, without additional synchronization or off-chip memory access.

By leveraging cluster level communication primitives, we design a fused decoding dataflow. As illustrated in Algorithm~\ref{alg:llama_fusion}, the dataflow is parallel in the number of attention heads. Each head corresponds to a cluster of $N = 2^k$ thread blocks ($k \leq 4$), where each block is assigned a rank $b \in [0, N-1]$. Within a cluster, thread blocks partition the hidden dimension during the linear projection stage and the KV cache sequence length during the attention stage. Each cluster processes a tile $H_b$ of the input hidden states and computes the corresponding output tile $O_b$ after the attention. In this algorithm, $B$ denotes the batch size, $h$ is the head dimension, $d$ is the hidden dimension and $s$ is the sequence length, which is partitioned across the thread blocks. 





==> sections/evaluation.tex <==
\section{Evaluation}
\paragraph{Experimental Setup} We evaluate ClusterFusion on an NVIDIA Tesla H100 SXM5 80GB GPU. For the end-to-end evaluation, all inputs are in FP16 precision, and the context length varies from 1K to 16K. We set the batch size to 1; results of multi batch are presented in the appendix. All experiments are conducted using PyTorch $2.5.1$ and CUDA $12.4$.

\paragraph{Baselines} We compare ClusterFusion with four state-of-the-art LLM deployment frameworks: SGLang $0.4.3$.post2, vLLM $0.6.4$.post1, TensorRT-LLM $0.18.0$, and MLC-LLM $0.20$.dev0. These frameworks often rely on manually optimized kernel libraries such as CUTLASS, FlashAttention, and FlashInfer, or use compiler-generated kernels by Triton or TVM. For all baselines, we adopt the best configurations recommended in their official documentation, which incorporate optimizations such as CUDAGraph and Torch.Compile. Performance metrics are collected using NVIDIA Nsight Systems.

\paragraph{Models} ClusterFusion is evaluated on two representative LLMs: Llama2-7B and DeepSeek-V2-Lite, both based on the Transformer architecture. Llama2-7B adopts standard Multi-Head Attention (MHA) mechanism, while DeepSeek-V2-Lite employs Multi-head Latent Attention (MLA) and Mixture-of-Experts (MoE) for FFN modules. These models differ in hidden dimensions, attention head dimensions, and number of attention heads.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/e2e-llama.pdf}
        \caption{Llama2-7B}
        \label{fig:e2e-llama}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/e2e-deepseek.pdf}
        \caption{DeepSeek-V2-Lite}
        \label{fig:e2e-deepseek}
    \end{subfigure}
    \caption{Time per output token (TPOT) of Llama2-7B and DeepSeek-V2-Lite on H100 GPU.}
    \label{fig:e2e}
\end{figure}

\subsection{End-to-End and Core Module Evaluation}

We use time per output token (TPOT) as the metric for end-to-end evaluation. The results are presented in \Fig{fig:e2e}. For baselines, the results include both CUDA graph launch and kernel execution latency. In contrast, ClusterFusion incurs negligible kernel launch overhead and achieves lower kernel execution latency. With a cluster size of 4, ClusterFusion outperforms the best baseline by up to $1.38\times$ over Llama2-7B and $1.65\times$ over DeepSeek-V2-Lite across a range of sequence lengths. Specifically for DeepSeek-V2-Lite, ClusterFusion demonstrates particularly strong performance on short sequence lengths, and achieves performance comparable to the best baseline on long sequences. In contrast, SGLang and vLLM exhibit relatively stable end-to-end performance across different sequence lengths. This is because the MLA kernels they adopt maintain balanced latency regardless of sequence length, and the MoE module accounts for a significant portion of the total end-to-end latency, reducing the sensitivity to sequence length variation.

We also evaluate the performance of ClusterFusion under other cluster sizes, including 2, 8, and 16. The performance results are shown in \Fig{fig:cluster}, where C$2$ represents cluster size of 2, and so on. With a cluster size of 2, the overall parallelism is insufficient and it fails to fully utilize the hardware resources. Conversely, cluster sizes of 8 and 16 introduce increased interconnect latency and bandwidth contention, as more thread blocks within each cluster compete for shared communication channels. Additionally, the maximum SM occupancy decreases, limiting active core utilization, as illustrated in \Fig{fig:dsm}. Therefore, combining theoretical analysis with empirical observations, we conclude that a cluster size of 4 provides the optimal performance in our setting.

Compared to baseline frameworks such as SGLang, vLLM, and TensorRT-LLM, which adopt a kernel-by-kernel execution model based on hand-optimized libraries, ClusterFusion avoids frequent round trips between off-chip and on-chip memory and considers dataflow design at a larger scope, leading to more globally efficient execution. TensorRT-LLM exhibits higher latency partly due to suboptimal choices in CUTLASS kernel selection for GEMM and GEMV operations in our experimental settings. MLC-LLM, on the other hand, employs TVM-generated attention kernels, which tend to underperform compared to the specialized implementations adopted by other frameworks, particularly under long sequence lengths.

\begin{figure}[htbp]
    \centering
    \begin{minipage}[t]{0.38\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/cluster.pdf}
        \caption{TPOT comparison of ClusterFusion with different cluster sizes on Llama2-7B.}
        \label{fig:cluster}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.6\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/breakdown.pdf}
        \caption{Breakdown for the latency of a Transformer block of Llama2-7B and DeepSeek-V2-Lite.}
        \label{fig:breakdown}
    \end{minipage}
\end{figure}

\subsection{Breakdown Analysis}

We perform a breakdown analysis of the individual components within a Transformer block to illustrate the speedup achieved by ClusterFusion. As shown in \Fig{fig:breakdown}, the results are measured with a sequence length of 1K. Results for other sequence lengths are provided in the appendix.

For the linear and attention modules, ClusterFusion outperforms the best baseline, achieving speedups of up to $1.38\times$ and $2.28\times$ on Llama2-7B and DeepSeek-V2-Lite, respectively. ClusterFusion implements both the linear and attention modules within a single persistent kernel, eliminating the global barrier overhead present in the baseline and achieving better overall performance. For the FFN layers, ClusterFusion fuses the three GEMM operations with the intermediate element-wise activation and multiplication into a single kernel, storing intermediate results in on-chip shared memory. This approach achieves performance comparable to the state-of-the-art kernel library, CUTLASS, which is used in the baseline framework. In the representative element-wise operation RMSNorm, ClusterFusion achieves up to $1.56\times$ speedup with a cluster size of 2 over the best baseline, which is from the FlashInfer library. The performance gain is attributed to the dataflow of ClusterFusion that maps each batch to a cluster of more than one thread blocks. This dataflow design enhances overall parallelism, particularly under large hidden dimensions which is aligned with the scaling trend of modern large language models.

\begin{figure}[htbp]
    \centering
    \begin{minipage}[t]{0.4\linewidth}
        \vspace{0pt}  
        \centering
        \includegraphics[width=\linewidth]{figs/ablation.pdf}
        \caption{TPOT comparison of ClusterFusion with and without DSMEM.}
        \label{fig:ablation}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.58\linewidth}
        \vspace{0pt}  
        \centering
        \captionof{table}{Latency comparison of on-chip AllReduce and AllGather with DSMEM versus off-chip implementations without DSMEM.}
        \label{tbl:reduce_gather_latency}
        \vspace{2mm}
        \resizebox{\linewidth}{!}{%
            \begin{tabular}{ccccc}
                \toprule
                \textbf{Operation} & \textbf{Data Size ($KB$)} & \textbf{Off-chip ($\mu s$)} & \textbf{On-chip ($\mu s$)} & \textbf{Speedup} \\
                \midrule
                \multirow{4}{*}{\shortstack{\textbf{AllReduce}\\($cluster\_size=4$)}}
                    & 32  & 8.03  & 6.77  & 1.18$\times$ \\
                    & 64  & 9.01  & 6.61  & 1.36$\times$ \\
                    & 128 & 14.95 & 7.42  & 2.01$\times$ \\
                    & 256 & 22.44 & 9.17  & 2.44$\times$ \\
                \midrule
                \multirow{4}{*}{\shortstack{\textbf{AllGather}\\($cluster\_size=4$)}}
                    & 32  & 6.26  & 3.90  & 1.60$\times$ \\
                    & 64  & 6.27  & 4.12  & 1.52$\times$ \\
                    & 128 & 6.31  & 4.39  & 1.44$\times$ \\
                    & 256 & 6.61  & 4.15  & 1.59$\times$ \\
                \bottomrule
            \end{tabular}
        }
    \end{minipage}
\end{figure}

\subsection{Ablation Studies}

To demonstrate the importance of the on-chip interconnect leveraged in our dataflow design, we conduct a microbenchmark to evaluate the intra-GPU collective communication primitives introduced in \Sec{sec:api}. As shown in \Tbl{tbl:reduce_gather_latency}, the on-chip AllReduce and AllGather operations over DSMEM exhibit significantly lower latency across varying data transfer sizes.

We further perform ablation studies to compare ClusterFusion with and without DSMEM enabled. The experimental results are presented in \Fig{fig:ablation}. Across different sequence lengths, disabling DSMEM increases the time per output token (TPOT) by up to $33\%$. The size of the transferred intermediate results in this workload is theoretically around $217$ KB. According to our microbenchmark, the AllReduce primitive achieves a speedup of nearly $2.44\times$ at this data scale. However, its actual proportion of global memory traffic remains low, as it is overshadowed by the large model weights and KV cache. Therefore, this empirical observation is consistent with the theoretical analysis.


==> sections/related_work.tex <==
\section{Related Works}

\paragraph{LLM Operator-Level Optimizations}
Numerous researchs have explored operator-level optimizaitons for LLM inference. 
FlashAttention~\cite{fa1,fa2} fuses the entire Attention operation into a single memory-efficient kernel. Building on this, FlashDecoding~\cite{flashdec} extends parallelism to the KV cache sequence dimension during decoding. FlashDecoding++~\cite{fd++} proposes to determine the scaling factor based on statistics in advance and introduces FlatGEMM to represent the GEMM with a highly reduced dimension in decoding. FlashAttention-3~\cite{fa3} demonstrated that warp specialization and new hardware features such as asynchrony can have a significant impact on the Attention. FlashMLA~\cite{flashmla} design an efficient decoding Attention kernel for DeepSeek MLA architecture inspired by FlashAttention-3.
However, there optimizaitons adopt a block-isolated execution pattern. Due to the lack of structured communication across thread blocks, intermediate results are repeatedly written to and read from global memory, limiting opportunities for broader operator fusion and on-chip reuse. \proj{} explores a more general fusion space enabled by efficient cluster-scoped collective primitives.

\paragraph{LLM Algorithm-Level Optimizations}
Several studies focus on improving LLM inference efficiency through algorithmic changes. Techniques such as quantization~\cite{awq,vq-llm} and sparsification~\cite{nsa,moba} aim to reduce computational and memory overhead. Quantization compresses model weights and activations by converting high-bitwidth representations into lower-bitwidth ones, reducing arithmetic and memory costs. Sparsification increases the proportion of zero elements in weights or activations, enabling hardware to skip redundant computations. These techniques are orthogonal to our work. \proj{} does not modify the model workload but can complement these approaches by optimizing the underlying dataflow and kernel execution through structure and reusable primitives.

\paragraph{Systems on Inter-Core Connected Hardwares} The on-chip inter-core interconnect has also been adopted in alternative hardware platforms such as Graphcore IPU~\cite{graphcore} and Cerebras WSE~\cite{wse}. Several prior works have explored leveraging this capabilities to optimize deep learning workloads. T10~\cite{t10} is an end-to-end deep learning compiler targeting inter-core connected intelligence processors, with an emphasis on fine-grained modeling of data movement between cores. WaferLLM~\cite{waferllm}, on the other hand, is the first system to propose a LLM parallelism solution tailored for wafer-scale accelerators. Moreover, these systems are closely tied to custom hardware architectures that offer full inter-core connectivity or integrates inter-core communication mechanisms into specific operators like GEMM and GEMV. As such, their design assumptions do not translate well to modern GPU architectures like NVIDIA Hopper which remains the dominant platform for LLM inference deployment. \proj{} introduces cluster-scoped communication primitives which abstract common aggregation and reduction patterns and can be flexibly reused across different workloads.




 

% AWQ observes that weight channels vary in importance for performance, particularly emphasizing those aligned with input channels exhibiting outliers in activations. To enhance the preservation of critical weight channels, AWQ utilizes a reparameterization method. This technique selects reparameterization coefficients via grid search to minimize reconstruction errors effectively. VQ-LLM, an optimized code generation framework for vector quantization (VQ), consisting of codebook cache and codebook based compute engine. 
